Landscape Learning for Neural Network Inversion

Many machine learning methods operate by inverting a neural network at inference time, which has become a popular technique for solving inverse problems in computer vision, robotics, and graphics. However, these methods often involve gradient descent through a highly non-convex loss landscape, causing the optimization process to be unstable and slow. We introduce a method that learns a loss landscape where gradient descent is efficient, bringing massive improvement and acceleration to the inversion process. We demonstrate this advantage on a number of methods for both generative and discriminative tasks, including GAN inversion, adversarial defense, and 3D human pose reconstruction.

==> Table_bk.tex <==

%%%Our result backup
\begin{table}[]
\centering
\begin{tabular}{llcccc|cccc}

\toprule
% \multicolumn{8}{c}{\textbf{Adversarial Attack (results not entered yet)}} \\ \midrule
& \multicolumn{4}{|c|}{Adversarial Robust Accuracy}  & \multicolumn{4}{c}{Clean Accuracy}  \\
\multicolumn{1}{l|}{Optimization Steps}                                  & \multicolumn{1}{l|}{0 step}                  & \multicolumn{1}{l|}{1 step}       & \multicolumn{1}{l|}{2 steps}      & \multicolumn{1}{l|}{5 steps}   & \multicolumn{1}{l|}{0 step}    & \multicolumn{1}{l|}{1 step}       & \multicolumn{1}{l|}{2 steps}      & \multicolumn{1}{l}{5 steps}   \\ \midrule
% \multicolumn{1}{l|}{Undefended Baseline} & 0.00 & 1.70 & 3.30 & 6.10 & & 89.9 & 87.8 & 85.1  \\
% \multicolumn{1}{l|}{Undefended Ours}     & 0  &  16.33 & 16.99 & 17.64  & & 20.54 & 23.1 & 20.67\\     
% \midrule
\multicolumn{1}{l|}{Undefended Baseline} & 0.00 & 1.70 & 3.30 & 6.10 & & 89.9 & 87.8 & 85.1  \\
\multicolumn{1}{l|}{Undefended Ours}     & 0  &  16.33 & 16.99 & 17.64  & & 20.54 & 23.1 & 20.67\\     
\midrule
\multicolumn{1}{l|}{AWP Baseline \cite{AWP}} & 35.61 & 39.54 & 42.81 & 44.96 & & 87.73 & 86.9 & 85.83   \\
\multicolumn{1}{l|}{AWP Ours}     & 35.61 & 51.39 & 51.67 & 51.05 & & 74.89 & 78.26 & 80.86      \\     
\midrule
\multicolumn{1}{l|}{MART Baseline \cite{MART}} & 35.66 & 39.77 & 42.5 & 45.42 & & 74.70 & 78.20 & 80.82   \\
\multicolumn{1}{l|}{MART Ours}     &    35.66 &  51.77 & 51.77 & 50.96 & & 87.76 & 87.26 & 87.01 \\     
\midrule
\multicolumn{1}{l|}{SemiSL Baseline \cite{unlabeled}} & & 34.53 & 37.27 & 40.93 & &    \\
\multicolumn{1}{l|}{SemiSL Ours}     &       \\   
\bottomrule

\end{tabular}
\caption{Discriminative Model. Defending $L_2=256/255$ norm bounded attacks with self-supervised optimization. We perform 200 steps of PGD attack~\cite{madry2017towards} with a step size of $64/255$. We use the state-of-the-art defense for unforeseen attacks proposed by \cite{mao2021adversarial}, which is an optimization based defense that restore the performance for self-supervision task at inference time.}
\label{tab:attack}%
\end{table}
